Encodings of Observable Subalgebras

Simulating complex systems remains an ongoing challenge for classical computers, while being recognised as a task where a quantum computer has a natural advantage. In both digital and analogue quantum simulations the system description is first mapped onto qubits or the physical system of the analogue simulator by an encoding. Previously mathematical definitions and characterisations of encodings have focused on preserving the full physics of the system. In this work, we consider encodings that only preserve a subset of the observables of the system. We motivate that such encodings are best described as maps between formally real Jordan algebras describing the subset of observables. Our characterisation of encodings is general, but notably holds for maps between finite-dimensional and semisimple $C^{*}$-algebras. Fermionic encodings are a pertinent example where a mathematical characterisation was absent. Our work applies to encodings of the the full CAR algebra, but also to encodings of just the even parity sector, corresponding to the physically relevant fermionic operators.

==> dump.tex <==
\section{Old def motivation}

This work considers simulation where only part of the target system is reproduced in the simulator system. 
This framework is significantly less restrictive than demanding that the entire physics is reproduced as in \cite{Cubitt2019, Apel2023}. In many ways, considering just a subset is more natural and physically motivated since, in performing an analogue simulation, often only a small part of the system is of interest. 

We will nevertheless demand a strong form of simulation where the all measurement outcomes of the simulated observables are required to be reproduced. This means that the set of eigenvalues for an observable of and its simulated counterpart must be the same, while degeneracies and eigenvectors are free to differ, ensuring that all measurement outcomes for a target observable can be reproduced in some state of the simulator system.
Taking the Hamiltonian itself to be part of the set of simulated observables of interest is sufficient to reproduce all thermal properties and time dynamics of the target in the simulated system \cite{Cubitt2019}. 

This leads to the questions of what is the right set which should be preserved mathematically, and what are the the additional constraints that a map and simulator system must satisfy in order to obey usual quantum mechanics.
Note that for any observable $A$ of a quantum mechanical system, one can define the observable $\lambda A \in \mathcal{O}$ for $\lambda \in \mathbb{R}$ as the observable obtained by rescaling the measurement apparatus associated to $A$.
By a similar argument, one sees that the observable $A^{m}$ may be interpreted as the observable associated with taking the $m$th power of the results obtained after measuring $A$, so that the observable product $A^{m} A^{n} \equiv A^{m+n}$ is well defined.

Given two observables $A$ and $B$, one may also interested in calculating the expected value of the quantity $\lambda A + \mu B$ for some scalars $\mu, \lambda \in \mathbb{R}$ which are not necessarily dimensionless.
A crucial example of an observable which is the sum of two other observables is a Hamiltonian $H= \lambda p^{2} + \mu x^{n}$, where $p$ and $q$ are the momentum and position operators respectively. 

One is also interested in calculating the uncertainty $\Delta A$ of an observable $A$ in the state $\omega$, which can be understood as the quantum mechanical equivalent of the error. Writing the expectation value of $A$ in the state $\omega$ as $\omega(A)$, we can define the uncertainty as

\begin{equation}
    \Delta A = \omega(A^{2}) - (\omega(A))^{2}
\end{equation}

Since this must be well-defined even if the observable of interest is sum of two other observables, we must define the product of two non-equal observables. In the Dirac formulation of quantum mechanics, a quantum mechanical observable is a bounded self-adjoint operator on a Hilbert space. This justifies defining the product $B \circ C= \frac{1}{2}(B C+C  B)$ (called the Jordan product) in terms of the associative matrix multiplication, since the condition $( B \circ C)^{\dagger} = ( B \circ C)$ is immediately satisfied. \footnote{The factor of $1/2$ is there to ensure that under the definition the powers of an observable in this new product coincide with those as defined in the Dirac formulation.}
\ha{I think maybe the motivation for the jordan algbra being that we already have powers and addition so it just follows from combining them is a good one to add in maybe?}

We therefore define the algebra of a single observable as all real linear combinations and Jordan products of the observable. Similarly, for multiple observables, we consider the set of all real linear combinations and Jordan product of the set. It is easy to see that this forms a Jordan algebra (see \cref{appen C*} for more details) which is a Jordan subalgebra of the full algebra of observables. If we further restrict the algebras to satisfy the condition of being formally real, we arrive (for finite dimensional systems) at the definition of a special JB algebra. Such algebras are always guaranteed to be semisimple (see \cref{JordanvnWigner})\footnote{ Here we are using the fact that, for finite dimensional algebras, a special Jordan algebra is a JB algebra if and only if it is formally real (see \cite{jordanoalgebrasHancheStormer} for technical details). 
} %which has abundant discussions in the literature%, and was initially proposed by Jordan in order to generalise quantum mechanics in a way which could be applied to nuclear and relativistic phenomena. 

\begin{defn}[Special JB Algebra]\label{specialJBdefn} A special JB algebra is a special real Jordan algebra $A$ equipped with a complete norm, $\forall$ $a,b \in A$ satisfying 
\begin{enumerate}
    \item $\norm{a \circ b} \leq \norm{a} \norm{b}$;
    \item $\norm{a^{2}}=\norm{a}^{2}$;
    \item $\norm{a^{2}} \leq \norm{a^{2}+b^{2}}$.
\end{enumerate}
\end{defn}

It is clear from asserting measurement outcomes are preserved that we must demand that any simulation map be spectrum preserving. As well as spectrum preserving, we enforce the simulation map to be convex.
Operationally, a convex combination of observables corresponds to selecting an observable at random from the ensemble of observables according to some probability distribution, measuring that observable, and reporting the outcome. Constraining the simulation map to be convex is motivated by assuming that taking a probabilistic combination of simulated observables or considering the probabilistic combination as a new observable is indistinguishable. 
Hence formally, we will take a simulation of a subset of observables to be described by a map satisfying these two experimentally motivated conditions.

Since we are interested in spectrum preserving maps between now algebras and subalgebras of observables, we mathematically arrive at the following definition of a simulation map: 

\begin{defn}[Simulation map]\label{defn sim map}
    A map $\gamma: A \rightarrow B$ where $A$ and $B$ are two finite-dimensional special JB algebras, is a \emph{simulation map} if for all $a,a_1,a_2\in A$ and all $\lambda\in[0,1]$
    \begin{enumerate}[(i.)]
        \item $\textup{spec}[\gamma(a)] = \textup{spec}[a]$
        \item $\gamma(\lambda a_1 + (1-\lambda) a_2) = \lambda \gamma(a_1) +(1-\lambda)\gamma(a_2)$
    \end{enumerate}
\end{defn}

\section{Characterisation of simulation maps}\label{sect characterise}

Complex numbers and non-Hermitian operators have become integral to the study of quantum mechanics. However, it is much harder to make well-motivated assumptions about simulations in these cases. 
To avoid over assuming, \cref{defn sim map} acts between JB algebras where elements correspond to observables and therefore properties of maps on these objects can be motivated physically. 
A finite dimensional special JB algebra $A$ is necessarily contained in an associative algebra $\mathcal{A}$.
Our first step is to connect to more familiar associative algebras (such as $C^{*}$-algebras, of which the CAR algebra is an example) by extending the simulation map to the encompassing associative algebras.
\ha{Is the matrix algebra an example of a c star? If so think this could be a better example here maybe?}
The only assumption on this extended map is that its action on the self-adjoint elements of the associative algebra (the observables) is that of a simulation map as described in \cref{defn sim map}.
A priori the action of the extended map on non-symmetric elements is unconstrained.

%\ma{Can edit below to associative complex algebra to avoid c* algebra faff if we want?}

\begin{defn}[Extended simulation map]\label{defn ex sim map}
    Consider a simulation map $\gamma: A \rightarrow B$ where $A$ and $B$ are two finite-dimensional special JB algebras, and let $\mathcal{A}$ ($\mathcal{B}$) be the associative algebra in which $A$ ($B$) is contained.
    An extended simulation map $\Gamma: \mathcal{A}\mapsto \mathcal{B}$ has action consistent with $\gamma$ on symmetric elements, $\Gamma(a) = \gamma(a)$ for all $a \in A$.
\end{defn}

We first show that extended simulation maps are uniquely determined by the original simulation map, and therefore considering the mathematical form of $\Gamma$ instead of $\gamma$ introduces no ambiguity (\cref{lm:extended}).
Then, combining results from the associative algebra literature, \cite{jordanoalgebrasHancheStormer, mccrimmon, jordanVNWigner, Martindale, JacobsonandRickart}, we prove that extended simulation maps can be characterised. 
The first case considered is that of a simulation map $\gamma: A \mapsto B$ where $A$ is a simple JB algebra. This includes the case where all observables are simulated and $A \cong \text{Herm}_n$.

\begin{thm}[Characterisation of simple simulation map]\label{thm: simple map charac}
    Given a simulation map $\gamma: A \rightarrow B$, where $A$ is a simple algebra, and $B$ is a semisimple algebra, the extended simulation map $\Gamma: \mathcal{A}\rightarrow \mathcal{B}$ is completely characterised (up to unitary equivalence) by
    \[  \Gamma= \oplus_{i} \Gamma^{p_{i},q_{i}}(\alpha)= \oplus_{i} (\alpha^{\oplus p_{i}} \oplus \bar{\alpha}^{\oplus q_{i}}) \] 
    for all $\alpha\in\mathcal{A}$ and $p_{i},q_{i} \in \mathbb{N}_{0}$ such that $p_{i}+q_{i} = m_{i}/n$ where $\textup{dim}(\mathcal{A}) = n$, $\textup{dim}(\mathcal{B}_{i}) = m_{i}$. 
%    Given a simulation map $\gamma: A \rightarrow B$, where $A$ is a simple algebra, the extended simulation map $\Gamma: \mathcal{A}\rightarrow \mathcal{B}$ is completely characterised by
   % \[\Gamma^{p,q}(\alpha)= U(\alpha^{\oplus p} \oplus \bar{\alpha}^{\oplus q}) U^{\dagger}\] 
 %   for all $\alpha\in\mathcal{A}$ and any $p,q \in \mathbb{N}_{0}$ such that $p+q = m/n$ where $\textup{dim}(\mathcal{A}) = n$, $\textup{dim}(\mathcal{B}) = m$ and any $U \in \mathcal{B}$ such that $U U^\dagger = U^\dagger U= \mathds{1}$.
\end{thm}

The resulting form reduces to that found in \cite{Cubitt2019} in the cases where $B$ is a simple algebra. When $B$ is semisimple, the However, here we are interested in understanding the nature of encodings of semi-simple algebra $A$ can be embedded into different ideals of $B$, and with different multiplicitiess. Recall that sSemi-simple algebras arise in quantum mechanics when there are super-selection rules in the system, that is, rules which do not allow certain superpositions. In such systems, different super-selection sectors correspond to different summands in the algebra. 

An important example of a system with super-selection rules is a system with bosons and fermions. 

To relate to fermionic mappings, recall that, in fermionic systems, the observables of the system are self-adjoint operators $p_{i},q_{j}$ in a unital associative algebra $\mathcal{A}$ with involution satisfying $p_{k}p_{j}+p_{j}p_{k}= 2 \delta_{jk} 1$ and $p_{k}q_{j}+q_{j}p_{k}=0$. Fermionic systems are however often (equivalently) defined by introducing the operators $a_{k}= \frac{1}{2}(q_{k}+ip_{k})$ which imply the equations $a_{j}a_{k}+a_{k}a_{j}= 2 \delta_{jk}$ and $a_{j}a_{k}+a_{k}a_{j}= 2 \delta_{jk}$. One can easily verify that this algebra contains a set of matrix units, implying that the algebra is a $C^{*}$ algebra isomorphic to the simple algebra $M_{2^{n}}(\mathbb{C})$ in the standard way (see \cite{arvesoninvitation, JacobsonandRickart}). 


Since the observables in the $C^{*}$ algebraic description of fermions still correspond to the JB algebra of observables we have considered above, the theorem above applies to fermionic encodings. This can be seen as a consequence of the fact that every finite dimensional JB algebra is isometrically isomorphic to a Jordan subalgebra of a $C^{*}$ algebra (see \cite{jordanoalgebrasHancheStormer} for technical details). In this sense, the map above can be seen as a $C^{*}$-homomorphism, or, more precisely, a faithful representation of the CAR algebra. It is then easy to see how for example the Jordan-Wigner transformation \cite{JordanWigner} fits into this framework. As a corollary of our result, we characterise encodings of one semisimple algebra into another. 

\begin{col}[Characterisation of semisimple simulation map]\label{col: semisimple}
     Given a simulation map $\gamma: A \rightarrow B$, the extended simulation map $\Gamma: \mathcal{A}\mapsto \mathcal{B}$ is completely characterised (up to unitary equivalence) by
    \[\Gamma(\alpha)= \left(\bigoplus_{j} ( \alpha_{j})^{\oplus p_{ij}} \oplus ( \bar{\alpha}_{j})^{\oplus q_{ij}} \right) \]
    for all $\alpha= \alpha_{1} + ...+ \alpha_{i}+ ...+\alpha_{m}\in\mathcal{A}$ in $\mathcal{A} \cong \mathcal{A}_{1} \oplus ...\oplus \mathcal{A}_{i}... \oplus \mathcal{A}_{m}$ and $\mathcal{B} \cong \mathcal{B}_{1} \oplus ... \oplus \mathcal{B}_{i} ... \oplus \mathcal{B}_{n}$. 
    For some $\{p_{ij}\},\{q_{ij}\} \in \mathbb{N}_{0}$ such that $ (p_{ij}+q_{ij}) n_i= m_j$ where $\textup{dim}(\mathcal{A}_{i}) = n_{i}$, $\textup{dim}(\mathcal{B}_{i}) = m_{i}$, and the integers $p_{ij},q_{ij}$ denote the multiplicities of the embeddings of the $j$th summand of $\mathcal{A}$ into the $i$th summand of $\mathcal{B}$.
    %Given a simulation map $\gamma: A \rightarrow B$, any extended simulation map $\Gamma: \mathcal{A}\mapsto \mathcal{B}$ is completely characterised by
    %\[\Gamma^{\{p_i\},\{q_i\}}(\alpha)= U\left(\bigoplus_{i=1}^g (\epsilon_i\circ \alpha)^{\oplus p_i} \oplus (\epsilon_j\circ \bar{\alpha})^{\oplus q_i} \right)U^*\]
    %for all $\alpha\in\mathcal{A}$, where $\mathcal{A} \cong M_{n_1}(\mathbb{C})\bigoplus \dots \bigoplus M_{n_g}(\mathbb{C})$ and $\mathcal{B} \cong M_{m_1}(\mathbb{C})\bigoplus \dots \bigoplus M_{m_h}(\mathbb{C})$ and $\epsilon_i$ denotes the canonical surjection onto the $i$'th summand of $\mathcal{A}$.
    %For some $\{p_i\},\{q_i\} \in \mathbb{N}_{0}$ such that $\sum_{i=1}^{g} (p_i+q_i) n_i= \sum_{j=1}^h m_j$ and any $U \in \mathcal{B}$ such that $U U^* = U^* U= \mathds{1}$.
\end{col}

The key difference between \cref{thm: simple map charac} and \cref{col: semisimple} is that in the semisimple case, each subalgebra may be embedded in different subspaces of the algebra $B$, and with different degeneracies. 
\pagebreak
    
    
    
    
    EXPLAIN
    
    and obtain that $\Phi(a)=a^{\oplus q} \oplus \bar{a}^{\oplus q'}$ for some $q, q' \in \mathbb{N}_{0}$. Since this is a non-degenerate representation of $A$, by \cite{cstaralgebrasbook} corollary III.1.2, unitary equivalence follows. 
    \todo{Discuss with Harriet if this needs further explanation}
    \ha{Would like to spell out the last two sentences more to end up at a form the same as in the result statement}

         %We will show that if $\varphi$ is a unital $*$-homomorphism of $\mathcal{A}$ into $\mathcal{B}$, then $\varphi$ is determined up to unitary equivalence in $\mathcal{B}$.
    %Whereas $\phi$ is a Jordan homomorphism, \cref{lm:extended} gives that the extended simulation map $\Phi$ that is uniquely determined by $\phi$ is a unital associative homomorphism.
    %$Consider the canonical surjection $\epsilon_{i}$ onto the $i$th summand of 
    %$\mathcal{B}$, i.e. $\epsilon_i: \mathcal{B} \mapsto M_i(D)$ for some division ring $D$.
    %Then $\epsilon_{i} \circ \Phi: \mathcal{A} \rightarrow M_{i}(D)$  is a unital homomorphism between simple algebras.
    %Therefore, again by Schur's lemma $\epsilon_{i} \circ \Phi$ is either the zero homomorphism or an isomorphism.
    %This can be lifted to a $*$-homomorphism (satisfying the additional condition $ \epsilon_{i} \circ \varphi(a^{*})= (\epsilon_{i} \circ \varphi(a))^{*}$) $\iff$ $\phi(ib)=\pm i \phi(b)$ where $b$ is self-adjoint. It is clear that this choice does not affect the spectrum preserving properties of $\varphi$ for self-adjoint elements. Repeating the argument for each summand of $B$, the statement follows, with unitary equivalence being a direct consequence of the representation theory of finite dimensional $C^{*}$ algebras (see \cite{cstaralgebrasbook} Corollary III$.1.2$).

        Suppose that $\varphi$ is a unital $*$-homomorphism of $\mathcal{A}$ into $\mathcal{B}$. Then $ \varphi_{i} \equiv \epsilon_{i} \circ \varphi : \mathcal{A} \rightarrow M_{n_{i}}$ is a unital homomorphism from $A$ into the simple algebra $M_{n_{i}}(\mathbb{C})$, and is therefore [LIKE ABOVE].
    Using that $\varphi \cong \oplus_{i} \varphi_{i}$ we see that 
    
    of the form $\epsilon_{i} \circ \varphi (a) = a^{\oplus q} \oplus \bar{a}^{\oplus q'}$ for some $q, q' \in \mathbb{N}_{0}$. We repeat the argument for each summand of $\mathcal{B}$ and use that $\epsilon= \oplus_{i} \epsilon_{i}$. Unitary equivalence once again follows from \cite{cstaralgebrasbook} corollary III.1.2. 

    %By \cite{operatoralgebrasbook} proposition II.3.2.3, every element of a $C^{*}$ algebra can be written as the product of a self-adjoint element and an element which is not self adjoint. Writing $y=ab$ for $a=a^{*}$ and $b \neq b^{*}$, we use that $i\mathds{1}$ satisfies $b^{*}a=-ab$ 

%to evaluate $\Phi(ab-ab)= \Phi(ab+b^{*}a)=0$ which implies $\Phi(ab)^{*}=-$

%Observe that $\Phi(i \mathds{1})^{2}= -\mathds{1}$, so the operator $\Phi(i \mathds{1})$ has eigenvalues $\{\pm i\}$. Since $\Phi(i \mathds{1})$ is normal, it is unitarily diagonalisable, and since it is central, we can write $\Phi(\alpha)=  \Phi_{+}(\alpha) \oplus \Phi_{-}(\alpha) $ where the $\pm$ signs denote the action on the two invariant eigenspaces. 



substituting  $\alpha^{*}=\alpha^{-1}$ between steps. We see that $\Gamma(\alpha)^{*}\Gamma(\alpha^{*}) = \mathds{1}$

For any element $\alpha$ such that $\alpha^{*}=\alpha^{-1}$, we will apply the involution on the identity twice, substituting  in between. We have that $\Gamma(\alpha^{*})\Gamma(\alpha)=\mathds{1}$. Taking the involution once gives 


For a unitary, this is equivalent to $\Gamma(a^{*})=\Gamma(a)^{*} \iff \Gamma(\alpha^{*}) \Gamma(\alpha)^{*-1}=\mathds{1}$. For any unitary, we have $ \Gamma(a^{*}) \Gamma(a)=\mathds{1} \iff \Gamma(a)^{*} \Gamma(a^{*})^{*} = \mathds{1} \iff  \Gamma(a^{*})^{*-1} \Gamma(a)^{*-1} = \mathds{1} \iff \Gamma(a)^{*}= \Gamma(a^{*})^{*-1}$. Using $a^{*}=a^{-1}$ in the last implication, we conclude that the statement is true for all unitaries, and hence $\Gamma((i\mathds{1})^{*})=\Gamma(i\mathds{1})^{*}$. 


For a unitary, this is equivalent to $\Gamma(a^{*})=\Gamma(a)^{*} \iff \Gamma(\alpha^{*}) \Gamma(\alpha)^{*-1}=\mathds{1}$. For any unitary, we have $ \Gamma(a^{*}) \Gamma(a)=\mathds{1} \iff \Gamma(a)^{*} \Gamma(a^{*})^{*} = \mathds{1} \iff  \Gamma(a^{*})^{*-1} \Gamma(a)^{*-1} = \mathds{1} \iff \Gamma(a)^{*}= \Gamma(a^{*})^{*-1}$. Using $a^{*}=a^{-1}$ in the last implication, we conclude that the statement is true for all unitaries, and hence $\Gamma((i\mathds{1})^{*})=\Gamma(i\mathds{1})^{*}$. 



\subsection*{Fermionic encodings}

Mappings describing transformations between states of fermions and states of qubits are crucial for the simulation of fermionic systems \cite{fermiontoqubitcompact}, as well as useful for mapping complex hamiltonians of one type of system into simple, non-interacting Hamiltonians into the other \cite{NielsenJordanWigner}. Indeed, the importance of describing fermion to qubit mappings for digital simulation of quantum systems was already stressed by Feynman, who left the question of whether such mappings existed open in \cite{Feynmansimulation}. 

Multiple fermion to qubit mappings exist nowadays. Some examples include the Jordan-Wigner transformation, which does []; the Kitaev one, which does [], and the other one [], which does SOMETHING ELSE. All of these mappings preserve the set of fermionic observables, which is strictly smaller than the set of all observables for a system of equal dimension with no additional constraints. Since our framework focuses on mappings from fermionic hamiltonians into arbitrary Hamiltonians with no additional locality constraints, it is general enough to encompass the aforementioned mappings. 

Mappings describing transformations between states of fermions and states of qubits are crucial for the simulation of fermionic systems \cite{fermiontoqubitcompact}, as well as useful for mapping complex hamiltonians of one type of system into simple, non-interacting Hamiltonians into the other \cite{NielsenJordanWigner}. Indeed, the importance of describing fermion to qubit mappings for digital simulation of quantum systems was already stressed by Feynman, who left the question of whether such mappings existed open in \cite{Feynmansimulation}. 


\ma{NOW DESCRIBE THIS?}


%the CAR algebra is a semisimple algebra, this fits into our framework ,  MAKE POINT ABOUT HOW WE DON'T restrict LOCALITY of ENCODINGS mentioned in \cite{Harley2023}. 

In order to define the CAR algebra, we consider self-adjoint operators $p_{i},q_{j}$ in a unital associative algebra $\mathcal{A}$ with involution satisfying

\begin{equation}
    p_{k}p_{j}+p_{j}p_{k}= 2 \delta_{jk} 1
\end{equation}

\begin{equation}\label{pqdefn}
    p_{k}q_{j}+q_{j}p_{k}=0
\end{equation}

We will assume that $n$ is finite. The complex form of these relations is obtained by introducing the operators 

\begin{equation}
    a_{k}= \frac{1}{2}(q_{k}+ip_{k})
\end{equation}

which imply the equations

\begin{equation}
    a_{j}a_{k}+a_{k}a_{j}= 2 \delta_{jk}
\end{equation}

\begin{equation}
    a_{j}^{*}a_{k}+a_{k}a_{j}^{*}=1 \delta_{jk}
\end{equation}

which are called the canonical anticommutation relations. With $j=k$ in the second equation above, we obtain 

\begin{equation}
    a_{j}^{*}a_{j}+a_{j}a^{*}_{j}=1
\end{equation}

which one can use to note that $e_{j}^{*} \equiv a_{j}^{*}a_{j}$ and $e_{j} \equiv a_{j}a_{j}^{*}$ are orthogonal self adjoint idempotents, with each $a_{j}$ a nilpotent element of order two. 

Let $a_{1}, a_{2},...,a_{n}$ be a finite set of operators satisfying the canonical anticommutation relations. Then show that these are matrix units, prove isomorphism to matrix algebras, explain that this is a finite dimensional $C^{*}$ in the usual way... note that the observables are just the standard directs sums of pqs etc...(self adjoint elements in this matrix algebra) and everything else just goes through... 


Multiple fermion to qubit mappings exist nowadays. Some examples include the Jordan-Wigner transformation \cite{JordanWigner}, the map by Bravyi and Kitaev \cite{BravyiKitaev}, and the compact mapping of \cite{fermiontoqubitcompact}. Since our framework encompasses mappings from fermionic Hamiltonians into arbitrary Hamiltonians with no additional locality constraints, it is general enough to include the aforementioned mappings. 


After defining some notation, \cref{sect def sim} begins by motivating the definition of a simulation map between a subset of observables, which largely hinges on pinning down the correct algebraic structure to describe a simulated subset of observables.
\cref{sect characterise} characterises the simulation map for both a simple algebra into a semisimple algebras, and from semisimple algebras into arbitrary algebras, giving the main result.
Although the result is general, we then explore the $\mathrm{CAR}$  algebra to connect with fermionic encodings. 

 the algebra for $n$ fermionic degrees of freedom is a $C^{*}$ algebra isomorphic to $M_{2^{n}}(\mathbb{C})$, for which each fermionic degree of freedom generates a $2 \times 2$ matrix subalgebra (which is therefore simple) \cite{arvesoninvitation}. 


\section{even odd car}


However the even sector is a subalgebra (refer to a definition of subalgebra) and so we can consider encoding only this subalgebra. This could have advantage over encoding the full CAR algebra since a smaller algebra needs to be preserved leading to hope that fewer physical resources are required to simulate these even fermionic operators. 


There is additional new scope here as the even CAR subalgebra is semi-simple and so encodings of this subalgebra have the additional freedoms of our Thm ?. This means that we can take different degeneracies of the two (what are the blocks of a semisimple algebra called) in the encoding. The CAR alegbra is isomorphic to the Clifford algebra. While Clifford algebras are well studied in the literature our regime of interest (finitie dimensional systems with complex algebras) is less common amungst mathematicians (who prefer real algebras) and field physicists (who prefer infinite dimensions). That the even CAR subalgebra is semi simple can be shown by careful consideration of this literature. 
Our work does the lifting defining and characterising encodings of subalgebras, highlighting that in the case of fermionic encodings there is untapped potential in devloping 'even fermionic encodings' that only deal with the physically relevent even CAR subalgebra. It is also notable that since this algebra is semisimple it fits the more general mathematical characterisation than the simple CAR algebra. With these insights, our work leaves open the question of finding and analysing explicit examples of these even fermionic encodings.  




The CAR algebra is simple and so our Thm ?? applies and the above encodings all adhere to the mathematical form in eqn ?? The key differences arising between the choice of unitary. 
While CAR is simple, an interesting consideration is the parity sectors, dividing the algebra into a sector of even and odd parity. 
The even sector corresponds to operators where ? e.g. whereas the odd sector e.g.
One observes that many fermionic operators of physical interest e.g. the fermi-hubbard hamiltonian etc are all even operators. This is understood due to locality... leading to the even sector sometimes being referred to as the 'physically relevant algebra'

As CAR is simple, the parity opporator does not make CAR block diagonal (this can be understood as taking the product of two operators in the odd sector results in an even operator and so the odd sector is not closed).





Fermions are the group of particles that obey anticommutation relations the ubiquitous example are electrons
Electronic wavefunctions govern molecular interactions and material properties, therefore simulating fermionis is a key application of quantum computing.  
Generally quantum devices are constructed based on qubits, and so both for analogue and digital simulation an encoding is required to translate the Hamiltonian from fermionic annihilation and creation opperators to qubit opperations. 

Even thing is a universal set....


Algebraically, finite-dimensional systems of interacting fermions are described by the canonical anticommutation relations algebra (CAR algebra) the simple $C^{*}$ algebra defined by ...

DEFINED HERE






Algebraically the fermions are described by the CAR (cannonical anticommutation relations) algebra. Different encodings of CAR to systems of qubits exist (Jordan Wigner, Bravyi-Kitaev as well as local encodings). These map the full CAR algebra to a composite Hilbert space made up of qubits.


There is additional new scope here as the even CAR subalgebra is semi-simple and so encodings of this subalgebra have the additional freedoms of our Thm ?. This means that we can take different degeneracies of the two (what are the blocks of a semisimple algebra called) in the encoding. The CAR alegbra is isomorphic to the Clifford algebra. While Clifford algebras are well studied in the literature our regime of interest (finitie dimensional systems with complex algebras) is less common amungst mathematicians (who prefer real algebras) and field physicists (who prefer infinite dimensions). That the even CAR subalgebra is semi simple can be shown by careful consideration of this literature. 
Our work does the lifting defining and characterising encodings of subalgebras, highlighting that in the case of fermionic encodings there is untapped potential in devloping 'even fermionic encodings' that only deal with the physically relevent even CAR subalgebra. It is also notable that since this algebra is semisimple it fits the more general mathematical characterisation than the simple CAR algebra. With these insights, our work leaves open the question of finding and analysing explicit examples of these even fermionic encodings.  

However, here we note that by theorem \ma{THEOREM}, the encodings of the physically relevant algebra are fundamentally different. 

semi-simple and so encodings of this subalgebra have the additional freedoms of our Thm ?. This means that we can take different degeneracies of the two (what are the blocks of a semisimple algebra called) in the encoding.

One then sees that the observables for the fermionic system in the $C^{*}$ algebraic description form a JB algebra of observables as considered above, and hence the theorems described here apply to fermionic encodings. Since these maps can be seen as a $C^{*}$-homomorphism, one can see how mappings such as the Jordan-Wigner transformation \cite{JordanWigner} fit into this framework. As a corollary of our result, we may also characterise encodings between semisimple algebras. 

It is also notable that since this algebra is semisimple it fits the more general mathematical characterisation than the simple CAR algebra.


Todo:
\begin{enumerate}
    \item In notation and terminology add in text definition of subalgebra. And a subalgebra can be be a special JB algebrs
    \item Add some citations in about fermions and more intro about the CAR alegbra (move from previous section)
    \item add proper proof that even CAR is semi simple with reference (Maite) \ma{there is no proof, just reference}
    \item We outline whats mathematically possible for encoding different algebras, (maybe?) mention equipped with an encoding for even CAR could also have different degeneracies for even and odd if it was found ot be advantageous
\end{enumerate}


Clifford algebras are well studied in the literature, however our regime of interest (finite dimensional systems with complex algebras) is less common amongst mathematicians (who prefer real algebras) and field physicists (who prefer infinite dimensions).
The CAR algebra is isomorphic to the Clifford algebra \ha{maybe expand a tiny bit and just cite}.
We can use this relation to infer that the even CAR subalgebra is semi simple by careful consideration of this literature. \ha{add citations and the proper reasoning here}

OLD: 

In the previous section, we extended the notion of simulation maps from special JB algebras to the $C^{*}$ algebras that they are contained in. Conversely, it is straightforward to verify that, given a finite-dimensional $C^*$ algebra, the set of self-adjoint elements is always a special JB algebra. An advantage of extending the notion of encodings from special JB algebras to $C^{*}$ algebras as in the previous section is that the results are applicable to the canonical anticommutation (CAR) relations, the $C^{*}$ algebra which describes systems of interacting fermions. Understanding of fermionic encodings is of crucial importance for fields such as condensed matter and quantum chemistry, where electronic wavefunctions govern material properties and molecular interactions. 

For both analogue and digital simulation, where fermionic Hamiltonians are often simulated using qubits, an encoding is required to translate the Hamiltonian from fermionic annihilation and creation operators to qubit operators.
Several encodings of the canonical anticommutation relations in qubit systems exist, for example the Jordan-Wigner transformation \cite{JordanWigner} and the Bravyi-Kitaev encoding \cite{BravyiKitaev}. Encodings such as the Jordan-Wigner transformation map the full algebra of observables to a composite Hilbert space made up of qubits, and since the full CAR algebra is well-known to be a simple algebra, these encodings are characterised by applying theorem \ref{thm: simple map charac} to simple algebras.  %or after noting that every simple $C^{*}$ algebra is isomorphic to $M_{n}(\mathbb{C})$ for some $n \in \mathbb{N}$ . 

In the $C^{*}$ algebraic literature as well as in the quantum chemistry literature, the Hamiltonians of interest are restricted to the even subalgebra of the CAR algebra, which is often dubbed the `physically relevant algebra' \cite{bravyikitaevforelectrons, BravyiKitaev}. In this section we will note that, at least in principle, the encodings of the physically relevant algebra are fundamentally different and characterised by \cref{col: semisimple}. 

Fermionic systems are often defined in the physics literature by introducing annihilation and creation operators $a_{k}$ and $a^{*}_{k}$ such that $a_{j}^{*}a_{k}+a_{k}a_{j}^{*}= 2 \delta_{jk}\mathds{1}$ and $a_{j}a_{k}+a_{k}a_{j}= 0$\footnote{On the other hand they can be equivalently defined by self-adjoint operators $p_{i},q_{j}$ in a unital associative algebra with involution satisfying $p_{k}p_{j}+p_{j}p_{k}= 2 \delta_{jk} \mathds{1}$ and $p_{k}q_{j}+q_{j}p_{k}=0$ such that $a_{k}= \frac{1}{2}(q_{k}+ip_{k})$.}. In the $C^{*}$ algebraic literature, the $C^{*}$ algebra of fermions is defined by 

One can verify that this algebra contains a set of matrix units, implying that the algebra is a simple $C^{*}$ algebra isomorphic to the simple algebra $M_{2^{n}}(\mathbb{C})$ via a canonical embedding into a matrix ring (see \cite{arvesoninvitation, JacobsonandRickart, rowenringtheory}). Consider now the set of all operators in the above algebra which are products and linear combinations of an even number of creation and annihilation operators. It is easy to see that this is a subalgebra of the full $C^{*}$ algebra of fermions. In infinite dimensions, the even subalgebra is in fact isomorphic to the full algebra of fermions \cite{stormer1970even}. However, in the finite-dimensional case, this is not the case, for reasons we now explain.

Consider first the automorphism $\gamma$ on the CAR algebra which acts as $\gamma: a_{i} \mapsto -a_{i}$ for every generator and extend multiplicatively in the following way:   . It is clear that the even algebra is invariant under the action of $\gamma$. The automorphism $\gamma$ is a central idempotent in the even algebra (but not in the full algebra) and so the CAR algebra splits into $A= \gamma \mathcal{A} \bigoplus(1-\gamma) \mathcal{A}$ as a vector space but not as an algebra, whilst the even algebra $\mathcal{A}_{even}$ splits into $A_{even}= \gamma \mathcal{A}_{even} \bigoplus(1-\gamma) \mathcal{A}_{even}$ where  $\gamma \mathcal{A}_{even}$  and $(1-\gamma) \mathcal{A}_{even}$  are now subalgebras of $\mathcal{A}_{even}$ and the direct sum is as an algebra \footnote{Though these are standard arguments in the theory of algebras, ...}. Using well-known theorems in the representation of finite-dimensional algebras \cite{garling2011} , it follows that $A_{even} \cong $. Because of this, the encodings of the even algebra are characterised by \cref{col: semisimple}. 

Our work does the lifting defining and characterising encodings of subalgebras, highlighting that in the case of fermionic encodings there is untapped potential in developing `even fermionic encodings' that only deal with the physically relevant even CAR subalgebra. With these insights, our work leaves open the question of finding and analysing explicit examples of these even fermionic encodings.  
The major challenge remains of finding the unitaries in the encoding that map from the even CAR algebra to algebras of qubits.

.

Consider first the automorphism $\gamma$ on the CAR algebra which acts as 
\[
\gamma: a_{i} \mapsto -a_{i}
\]
for every generator and extend multiplicatively by defining
\[
\gamma(a_{i_1}a_{i_2}\cdots a_{i_k}) = (-1)^k\, a_{i_1}a_{i_2}\cdots a_{i_k}.
\]
It is clear that the even algebra is invariant under the action of $\gamma$. The parity operator, which implements the automorphism $\gamma$, is central in the even algebra (but not in the full algebra) and so the CAR algebra splits into 
\[
A = \gamma \mathcal{A} \oplus (1-\gamma) \mathcal{A}
\]
as a vector space but not as an algebra, whilst the even algebra $\mathcal{A}_{even}$ splits into 
\[
A_{even} = \gamma \mathcal{A}_{even} \oplus (1-\gamma) \mathcal{A}_{even},
\]
where $\gamma \mathcal{A}_{even}$ and $(1-\gamma) \mathcal{A}_{even}$ are now subalgebras of $\mathcal{A}_{even}$ and the direct sum is as an algebra

